Subdimensional Expansion for Multi-objective Multi-agent Path Finding

Conventional multi-agent path planners typically determine a path that optimizes a single objective, such as path length. Many applications, however, may require multiple objectives, say time-to-completion and fuel use, to be simultaneously optimized in the planning process. Often, these criteria may not be readily compared and sometimes lie in competition with each other. Simply applying standard multi-objective search algorithms to multi-agent path finding may prove to be inefficient because the size of the space of possible solutions, i.e., the Pareto-optimal set, can grow exponentially with the number of agents (the dimension of the search space). This paper presents an approach that bypasses this so-called curse of dimensionality by leveraging our prior multi-agent work with a framework called subdimensional expansion. One example of subdimensional expansion, when applied to A*, is called M* and M* was limited to a single objective function. We combine principles of dominance and subdimensional expansion to create a new algorithm named multi-objective M* (MOM*), which dynamically couples agents for planning only when those agents have to "interact" with each other. MOM* computes the complete Pareto-optimal set for multiple agents efficiently and naturally trades off sub-optimal approximations of the Pareto-optimal set and computational efficiency. Our approach is able to find the complete Pareto-optimal set for problem instances with hundreds of solutions which the standard multi-objective A* algorithms could not find within a bounded time.

==> contents/discuss.tex <==

\subsection{Relationship to M*}\label{sec:relation_to_mstar}
The MOMAPF problem, as defined in Sec.~\ref{sec:problem} generalizes the conventional (single-objective) MAPF: when $M=1$, the MOMAPF problem becomes a conventional (single-objective) MAPF problem and the solution set consists of only one solution with the optimal cost value. Similarly, the proposed MOM* algorithm can also be regarded as a generalization of M* to handle multiple objectives. Specifically, when $M=1$, MOM* solves (single-objective) MAPF in the following sense.
\begin{itemize}
    \item State comparison becomes ``$\leq$'' (no larger than) relationship between two scalar cost values.
    \item In every search iteration, a state with a non-dominated ($i.e.$ minimum) cost value in OPEN is popped, which guarantees that the first solution identified is the one with the minimum cost value (denoted as $C^*$).
    \item All candidate states in OPEN have cost no less than $C^*$ and are thus pruned in the sub-procedure that filters OPEN with $C^*$, which leads to the termination of the algorithm as OPEN becomes empty.
    \item Procedure DomBackProp and maintaining a set OPEN($v$)$\bigcup$CLOSED($v$) at each joint vertex $v \in \mathcal{V}$ are redundant when $M=1$ since there is only \emph{one} optimal path from $v_o$ to any $v \in \mathcal{V}$.
\end{itemize}

\subsection{Generalization to other objectives}

==> contents/outdated_result.tex <==


\graphicspath{{../contents/paper_fig/}}

\subsection{Experiment Setup and Heuristics}

We implemented both MOM* and NAMOA*~\cite{namoa} in Python. The NAMOA* serves as a baseline approach and is applied to the the joint graph $\mathcal{G}$ corresponding to agents to search for the entire set of Pareto-optimal solutions connecting $v_o$ and $v_f$. Both algorithms are compared on a computer with a CPU of 2.5 GHz Intel Core i7 and 16GB RAM. We tested with different four-connected grids, which will be elaborated later.
In each grid, every agent has a cost vector $a^i$ of length $M$ (the number of objectives) and every edge in the grid has a scaling vector $b$ of length $M$. The elements in both $a^i, \forall i\in I$ and $b$ are randomly sampled from integers in $[1,10]$. The cost vector for agent $i$ to go through an edge is the element-wise product of $a^i$ of agent $i$ and $b$ of that edge. 

In the implementation, to compute heuristics $h(v), v\in \mathcal{V}$, we first run single-agent NAMOA* search backwards from $v^i_f$ to all other vertices in the (individual) graph $G$, which computes the set of all Pareto-optimal cost vectors $\{g^i_*(\pi^i(v^i_f,u))\}$ of paths from $v^i_f$ to $u \in V$ for agent $i \in I$. Then, for each vertex $u\in V$, the element-wise minimum over every cost vectors in $\{g^i_*(\pi^i(v^i_f,u))\}$ forms a cost vector $h^i(u)$ which underestimates the cost vectors of any path from $u$ to $v^i_f$. Finally, the heuristic value of a joint vertex $v\in \mathcal{V}$ is computed by $h(v)=\Sigma_{i\in I} h^i(v^i)$, where $v^i$ is the individual vertex contained in $v$ for agent $i$. This heuristic is computed by a pre-processing step in both MOM* and NAMOA* implementation in our tests.

\subsection{NAMOA* vs MOM*}

\begin{figure}[htbp]\label{fig:random_grid_result}
	\centering
	%	\vspace{-4mm}
	\begin{minipage}{.15\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{grids_0p2_0.png}
		\includegraphics[width=1.0\linewidth]{grids_0p2_1.png}
%		\vspace{-4mm}
		%		\caption{Average success rate of finding the entire Pareto-optimal set within one minute.}
		% 		\vspace{-4mm}
		\label{fig:random_grid_sample}
	\end{minipage}%
	\begin{minipage}{.35\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{momapf_10x10_obst0p2_all_sol_rate_namoa_mom_inflated.png}
		\vspace{-4mm}
		%		\caption{Average success rate of finding the entire Pareto-optimal set within one minute.}
		% 		\vspace{-4mm}
		\label{fig:0p2_all_rate}
	\end{minipage}%
	\caption{Two of the five grids used in the test are plotted on the left. On the right, the average success rates about finding the entire Pareto-optimal set of NAMOA*, MOM* and inflated MOM* within one minute are shown.}\label{fig:0p2_all}
	%\end{figure}
	%
	%\begin{figure}
	\centering
	\vspace{4mm}
	\begin{minipage}{.5\textwidth}
		\centering
		\includegraphics[width=0.9\linewidth]{momapf_self-10x10_heu_weight_namoa_numexpd_runtime_boxplot.png}
		\vspace{-2mm}
		\caption{Left plot: the spread of run time for NAMOA*. Right plot: the spread of number of states expanded for NAMOA*.}
		% 		\vspace{-4mm}
		\label{fig:10x10_namoa}
	\end{minipage}%
	%	 \hspace{5mm}
	\vspace{4mm}
	\begin{minipage}{.5\textwidth}
		\centering
		\includegraphics[width=0.9\linewidth]{momapf_self-10x10_heu_weight_mom_numexpd_runtime_boxplot.png}
		\vspace{-2mm}
		\caption{Left plot: the spread of run time for MOM*. Right plot: the spread of number of states expanded for MOM*.}
		\label{fig:10x10_mom}
	\end{minipage}
	\vspace{4mm}
% 	\begin{minipage}{.5\textwidth}
% 		\centering
% 		\includegraphics[width=0.9\linewidth]{momapf_self-10x10_heu_weight_mom-w12_numexpd_runtime_boxplot.png}
% 		\vspace{-2mm}
% 		\caption{Left plot: the spread of run time for inflated (w=1.2) MOM*. Right plot: the spread of number of states expanded for inflated (w=1.2) MOM*.}
% 		\label{fig:10x10_momw12}
% 	\end{minipage}
\end{figure}

%\begin{figure}
%	\centering
%		\hspace{-3mm}
%		\includegraphics[width=.5\linewidth]{grids_0p2_0.png}
%		\hspace{-6mm}
%		\includegraphics[width=.5\linewidth]{grids_0p2_1.png}
%		\hspace{-6mm}
%		\includegraphics[width=.5\linewidth]{grids_0p2_2.png}
%		\hspace{-6mm}
%		\includegraphics[width=.5\linewidth]{grids_0p2_3.png}
%		\hspace{-6mm}
%		\includegraphics[width=.5\linewidth]{grids_0p2_4.png}
%		\hspace{-3mm}
%		\vspace{-3mm}
%		\caption{Test grids with 20\% random obstacles.}
%		\label{fig:grids}
%\end{figure}

We began our tests with five different 10 by 10 four-connected grids with 20\% random obstacles. % as shown in Figure \ref{fig:grids}. 
For each grid, 20 test cases were generated with random start and goal vertices for a set of $N$ agents with $N=2,4,\dots,12$ and we set the number of objectives $M=1,2,4$. For each test instance, we limit the search time of the algorithms to {\bf one minute}. We report the results on success rates, number of states expanded and run time distribution. Notice that run time includes both Pareto policies computation, which is a pre-processing step for MOM*, and MOM* search time. 

\paragraph{Success rate under bounded time:}
As shown in Figure \ref{fig:0p2_all}, MOM* achieves better success rates than NAMOA* in terms of finding the complete Pareto set. For NAMOA*, four agents is roughly the maximum number of agents that can be handled within a minute, since the success rates for $M=2$ and $M=4$ are lower than 10\%. MOM* achieves around 80\% and 50\% success rates for four agents with two and four objectives respectively. 

% \paragraph{MOM* vs inflated MOM*}
% MOM* achieves better success rates when the heuristic weight $w$ is inflated with a scalar larger than one, which allows MOM* trades off between computational efficiency and bounded sub-optimality. When $N=4$, inflated MOM* ($w=1.2$) achieves almost hundred percentage success rate for both $M=2$ and $M=4$ and when $M=4$, inflated MOM* almost doubles the success rate compared with the MOM* without inflation.

\paragraph{The size of Pareto-optimal set}
To get a better sense of the difficulty of the problem and the size of the Pareto-optimal set approximated with inflated heuristics, in Table \ref{table.m4sizes}, we listed the average and maximum number of Pareto-optimal solutions with four objectives ($M=4$) over all succeeded cases when the succeeded case count is more than 20. It's obvious that when the heuristic is not inflated ($w=1$), there is a large number (usually in hundreds) of Pareto-optimal solutions for problem instances which makes it burdensome to compute the entire Pareto-optimal set. By inflating the heuristic a little bit (with $w=1.2$), when there are two or four agents, MOM* almost reduces the size of the Pareto-optimal set by a factor of ten. As a result, MOM* trades off between the size of the sub-optimal Pareto-optimal sets computed and the computation time. We also want to point out the underlying bias in the table, as we can only count the number of Pareto-optimal solutions for succeeded cases and the succeeded cases typically have a smaller Pareto-optimal set compared with the failed cases. This explains why we didn't observe further growth in the size of Pareto-optimal set as the number of agents increases beyond four or six.

\begin{table}[htbp]
	\centering
	\begin{tabular}{ |c|c|c|c|c|c|c| } 
		\hline
		\multicolumn{7}{|c|}{M=4, w=1.0} \\
		\hline
		number of agents & 2 & 4 & 6 & 8 & 10 & 12 \\
		\hline
		number of succeeded cases & 100 & 49 & 10 & 2 & 0 & 0 \\ 
		\hline
		avg size of Pareto set & 36.7 & 70.96 & - & - & - & - \\ 
		\hline
		max size of Pareto set &333 & 391 & - & - & - & - \\
		%		\hline
		%		min size of Pareto set & 1 & 2 & - & - & - & - \\ 
		\hline
		\hline
		\multicolumn{7}{|c|}{M=4, w=1.2} \\
		\hline
		number of agents & 2 & 4 & 6 & 8 & 10 & 12 \\
		\hline
		number of succeeded cases & 100 & 96 & 76 & 30 & 13 & 3 \\ 
		\hline
		avg size of Pareto set & 3.91 & 7.71 & 7.13 & 7.90 & - & - \\ 
		\hline
		max size of Pareto set & 30 & 42 & 63 & 51 & - & - \\
		%		\hline
		%		min size of Pareto set & 1 & 1 & 1 & 1 & - & - \\ 
		\hline
	\end{tabular}
	\vspace{4mm}
	\caption{Sizes of Pareto sets with number of objectives $M=4$ and heuristic inflation $w=1.0,\;1.2$ for different numbers of agents. }
	\label{table.m4sizes}
\end{table}

\subsection{Grids from Online Benchmark}
To further corroborate the performance of MOM* and inflated MOM* with different heuristic inflation rates, we leveraged existing benchmark sets for MAPF \cite{stern2019multi} by selecting grids from different categories: room, maze and DAO game environment. We ran the algorithms with two objectives ($M=2$) and the cost vectors were generated with the same aforementioned procedure. We tested heuristic inflation rates $w=1.0, 1.1, 1.2, 1.5, 2.0$ with $N=2,4,6,\dots,20$ under \textbf{five minutes}.

\begin{figure}[htbp]\label{fig:bmk_room_result}
	\centering
	%	\vspace{-4mm}
	\begin{minipage}{.15\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{room-32-32-4.png}
		\vspace{-4mm}
		\label{fig:room_grid}
	\end{minipage}%
	\begin{minipage}{.35\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{momapf_room-32-32-4_all_sol_rate_heu_weight.png}
		\vspace{-4mm}
		\label{fig:room_all_rate}
	\end{minipage}%
	\caption{The room environment is plotted on the left. On the right, the average success rates about finding the entire Pareto-optimal set of MOM* and inflated MOM* (with different heuristic weights) within five minute are shown.}\label{fig:room_env_and_rate}
	\centering
	\vspace{2mm}
	\begin{minipage}{.5\textwidth}
		\centering
		\includegraphics[width=0.85\linewidth]{momapf_room-32-32-4_heu_weight_12_numexpd_runtime_boxplot.png}
		\vspace{-2mm}
		\caption{Left plot: the spread of run time for MOM* (w=1.2) for room environment. Right plot: the spread of number of states expanded for MOM* (w=1.2) for room environment.}
		% 		\vspace{-4mm}
		\label{fig:room_box_plot}
	\end{minipage}%
\end{figure}

\begin{figure}[htbp]\label{fig:bmk_maze_result}
	\centering
	%	\vspace{-4mm}
	\begin{minipage}{.15\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{maze-32-32-2.png}
		\vspace{-4mm}
		\label{fig:maze_grid}
	\end{minipage}%
	\begin{minipage}{.35\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{momapf_maze-32-32-2_all_sol_rate_heu_weight.png}
		\vspace{-4mm}
		\label{fig:maze_all_rate}
	\end{minipage}%
	\caption{The maze environment is plotted on the left. On the right, the average success rates about finding the entire Pareto-optimal set of MOM* and inflated MOM* (with different heuristic weights) within five minute are shown.}\label{fig:maze_env_and_rate}
	\centering
	\vspace{2mm}
	\begin{minipage}{.5\textwidth}
		\centering
		\includegraphics[width=0.85\linewidth]{momapf_maze-32-32-2_heu_weight_12_numexpd_runtime_boxplot.png}
		\vspace{-2mm}
		\caption{Left plot: the spread of run time for MOM* (w=1.2) for the maze environment. Right plot: the spread of number of states expanded for MOM* (w=1.2) for the maze environment.}
		% 		\vspace{-4mm}
		\label{fig:maze_box_plot}
	\end{minipage}%
\end{figure}


\begin{figure}[htbp]\label{fig:bmk_den312d_result}
	\centering
	%	\vspace{-4mm}
	\begin{minipage}{.15\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{den312d.png}
		\vspace{-4mm}
		\label{fig:den312d_grid}
	\end{minipage}%
	\begin{minipage}{.35\textwidth}
		\centering
		\includegraphics[width=1.0\linewidth]{momapf_den312d_all_sol_rate_heu_weight.png}
		\vspace{-4mm}
		\label{fig:den312d_all_rate}
	\end{minipage}%
	\caption{The DAO game environment is plotted on the left. On the right, the average success rates about finding the entire Pareto-optimal set of MOM* and inflated MOM* (with different heuristic weights) within five minute are shown.}\label{fig:den312d_env_and_rate}
	\centering
	\vspace{2mm}
	\begin{minipage}{.5\textwidth}
		\centering
		\includegraphics[width=0.85\linewidth]{momapf_den312d_heu_weight_12_numexpd_runtime_boxplot.png}
		\vspace{-2mm}
		\caption{Left plot: the spread of run time for MOM* (w=1.2) for the DAO game environment. Right plot: the spread of number of states expanded for MOM* (w=1.2) for DAO game environment.}
		% 		\vspace{-4mm}
		\label{fig:den312d_box_plot}
	\end{minipage}%
\end{figure}

From those tests (Figure \ref{fig:room_env_and_rate},\ref{fig:maze_env_and_rate},\ref{fig:den312d_env_and_rate}) we can observe that, in general, heuristic inflation effectively speeds up the algorithm. However, under various environments, the improvement by inflated heuristic can be very different. We also demonstrated the spead of run time as well as the number of states expanded in box plots (Figure \ref{fig:room_box_plot},\ref{fig:maze_box_plot},\ref{fig:den312d_box_plot}).
In addition, the size of the map affects the computational efficiency. In both room and maze like environment, the size of the grids is 32 by 32 while DAO game environment used is of size 65 by 81. During our tests, we observe that for large map, such as DAO we used, computing Pareto policies (via single-agent multi-objective search such as NAMOA*) for MOM* can be very burdensome: when there are more than 10 agents, computing Pareto policies may take up to five minutes (Figure \ref{fig:den312d_box_pol_time}). This further demonstrates the complexity of the problem.


\begin{figure}[htbp]
	\centering
	\begin{minipage}{.5\textwidth}
		\centering
		\includegraphics[width=0.6\linewidth]{momapf_den312d_heu_weight_12_poltime_boxplot.png}
		\vspace{-2mm}
		\caption{Time for computing Pareto policies.}
		% 		\vspace{-4mm}
		\label{fig:den312d_box_pol_time}
	\end{minipage}%
\end{figure}

